Quantum entanglement, sum of squares, and the log rank conjecture

For every $\epsilon>0$, we give an $\exp(\tilde{O}(\sqrt{n}/\epsilon^2))$-time algorithm for the $1$ vs $1-\epsilon$ \emph{Best Separable State (BSS)} problem of distinguishing, given an $n^2\times n^2$ matrix $\mathcal{M}$ corresponding to a quantum measurement, between the case that there is a separable (i.e., non-entangled) state $\rho$ that $\mathcal{M}$ accepts with probability $1$, and the case that every separable state is accepted with probability at most $1-\epsilon$. Equivalently, our algorithm takes the description of a subspace $\mathcal{W} \subseteq \mathbb{F}^{n^2}$ (where $\mathbb{F}$ can be either the real or complex field) and distinguishes between the case that $\mathcal{W}$ contains a rank one matrix, and the case that every rank one matrix is at least $\epsilon$ far (in $\ell_2$ distance) from $\mathcal{W}$. To the best of our knowledge, this is the first improvement over the brute-force $\exp(n)$-time algorithm for this problem. Our algorithm is based on the \emph{sum-of-squares} hierarchy and its analysis is inspired by Lovett's proof (STOC '14, JACM '16) that the communication complexity of every rank-$n$ Boolean matrix is bounded by $\tilde{O}(\sqrt{n})$.

==> macros-lp.tex <==
% paper-specific packages
% \usepackage{relsize}
% \usepackage[font=footnotesize]{caption}
% \usepackage{yfonts}

% abbreviations and paper-specific macros
\newcommand{\Id}{\mathop{\mathrm{Id}}\!\mathinner{}}
\newcommand{\pE}{\tilde {\mathbb E}}

\let\cL\relax
\DeclareMathOperator{\cL}{\mathcal L}
% this is a big hack but idk who's defining a bad version of argmax
\let\argmax\undefined
\DeclareMathOperator*{\argmax}{\arg \, \max}

\newcommand{\Span}{\mathsf{Span}}

% \newcommand*{\annotaterel}[2]{\stackrel{\scriptscriptstyle\text{#1}}{#2}}

% \DeclareUrlCommand\email{}

\newcommand{\tO}{\tilde O}
\newcommand{\tOmega}{\tilde \Omega}
\newcommand{\tTheta}{\tilde \Theta}
\newcommand{\Err}{\text{Err}}
\newcommand{\Lsym}{\text{Lsym}}
\newcommand{\Rsym}{\text{Rsym}}
\newcommand{\pEs}{{\pE^*}}
\newcommand{\Conn}{\mathsf{conn}}
\newcommand{\Connk}{k\mathsf{conn}}
\newcommand{\omegan}{{\left( \frac{\omega}{n} \right)}}
\newcommand{\omegasqn}{{\left( \frac{\omega^2}{n} \right)}}
\newcommand{\fR}{\mathfrak{R}}
\newcommand{\fI}{\mathfrak{I}}
\newcommand{\fV}{\mathfrak{V}}
\newcommand{\fU}{\mathfrak{U}}
\newcommand{\fD}{\mathfrak{D}}


% Paper specific macros
\newcommand{\iproduct}{g}


% Pravesh Kothari's Macros
% \newcommand{\pnote}[1]{\textcolor{blue}{\small{[Pravesh: #1]}}}
% \usepackage{appendix}
% \usepackage{amssymb}
 %\setlength\parindent{0pt}
% \usepackage{amsfonts}
% \usepackage{latexsym}
% \usepackage{amsmath}

% Ankur Moitra's Macros
\newcommand{\anote}[1]{\textcolor{green}{\small{[Ankur: #1]}}}

% \usepackage[T1]{fontenc}
% \usepackage{fullpage,appendix}
% \usepackage{dsfont}
%\usepackage[capitalize]{cleveref}

\usepackage{color}
% \usepackage{tikz}

\newcommand{\eqdef}{\stackrel{\textrm{def}}{=}}
\newcommand{\spn}{\S^{n-1}}
\newcommand{\tm}{\tilde{m}}
\newcommand{\ignore}[1]{}
\definecolor{corlinks}{RGB}{64,128,128}
\definecolor{cormenu}{RGB}{0,37,94}
\definecolor{corurl}{RGB}{0,46,91}

%\setlength{\parindent}{0in}
\newcommand{\on}{\{-1,1\}}
\newcommand{\1}{\mathds{1}}

\newcommand{\bkets}[1]{\left(#1\right)}
\newcommand{\sbkets}[1]{\left[#1\right]}
\newcommand{\braces}[1]{\left\{#1\right\}}
\newcommand{\ip}[2]{\langle #1, #2 \rangle}

\newcommand{\dcdf}{\mathsf{dcdf}}
\newcommand{\cor}{\mathsf{cor}}
\renewcommand{\P}{\mathcal{P}}
\newcommand{\BPP}{\mathbf{BPP}}
%\newcommand{\E} {\mathbb{E}}
\DeclareMathOperator*{\ex}{\mathbb{E}}
\DeclareMathOperator*{\pr}{\mathsf{Pr}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\size}{\mathsf{size}}
\newcommand{\erf}{ \mathsf{erf} }
\newcommand{\D}{\mathcal{D}}
%\renewcommand{\H}{\mathbb{H}}
%\newcommand{\cH}{\mathcal{H}}
%\newcommand{\G}{\mathcal{G}}
\newcommand{\V}{\mathcal{V}}
\renewcommand{\Top}{\mathsf{Top}}
%\newcommand{\N}{\mathbb{N}}
%\newcommand{\cN}{\mathcal{N}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\A}{\mathcal{A}}

%\newcommand{\cC}{\mathcal{C}}
%\newcommand{\C}{\mathcal{C}}
\newcommand{\W}{\mathcal{W}}
%\newcommand{\U}{\mathcal{U}}
%\newcommand{\cU}{\mathcal{U}}
\newcommand{\SO}{\mathsf{SO}}
\newcommand{\SU}{\mathsf{SU}}
% \newcommand{\sign}{\mathsf{sign}}
\renewcommand{\L}{\mathcal{L}}
\renewcommand{\O}{\mathcal{O}}
%\newcommand{\g}{\text{\frakfamily g}}
\newcommand{\g}{G}
%changing this to $G_{e}$ notation
\newcommand{\h}{\text{\frakfamily h}}
\newcommand{\CQ}{\mathsf{CQ}}
\newcommand{\tmu} {\tilde{\mu}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\tnu}{\tilde{\nu}}
\newcommand{\M}{\mathcal{M}}
% \newcommand{\card}[1]{\lvert#1\rvert}
% \newcommand{\norm}[1]{\lVert#1\rVert}
% \newcommand{\poly}{\mathsf{poly}}
% \newcommand{\Prob}{\Pr}
\renewcommand{\S}{\mathbb{S}}
\newcommand{\STAT}{\mathsf{STAT}}
%\newcommand{\CSTAT}{\mathsf{CSTAT}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor}
\newcommand{\zo}{\{0, 1\}}

%complexity classes
\newcommand{\Ppoly}{\mathsf{P/poly}}
\newcommand{\BPTIME}{\mathsf{BPTIME}}
\newcommand{\EXP}{\mathsf{EXP}}
\newcommand{\NP}{\mathsf{NP}}
\newcommand{\DTIME}{\mathsf{DTIME}}
\newcommand{\PSPACE}{\mathsf{PSPACE}}
\newcommand{\PH}{\mathsf{PH}}
\newcommand{\SIZE}{\mathsf{SIZE}}
\newcommand{\NEXP}{\mathsf{NEXP}}
\newcommand{\CSTAT}{\mathsf{CSTAT}}
\newcommand{\Maj}{\mathsf{MAJ}}
\newcommand{\cal}[1]{\mathcal{#1}}
% \newcommand{\eps}{\epsilon}
%\newtheorem{fact}{Fact}[section]
%
\newtheorem*{notation}{Notation}
\newtheorem*{untheorem}{Theorem}
%\newtheorem{theorem}[fact]{Theorem}
%\newtheorem{lemma}[fact]{Lemma}
%\newtheorem{corollary}[fact]{Corollary}
%\newtheorem{observation}[fact]{Observation}
%\newtheorem{proposition}[fact]{Proposition}
%\newtheorem{problem}[fact]{Problem}
%\newtheorem{claim}[fact]{Claim}
%\newtheorem{conjecture}[fact]{Conjecture}
%\newtheorem*{note}{Note}
%\newtheorem{remark}[fact]{Remark}
%\newtheorem{question}{Question}
%\theoremstyle{definition}
%\newtheorem{definition}[fact]{Definition}
%

%
%\floatstyle{plain}
%\newfloat{myalgo}{tbhp}{mya}
%
%\newenvironment{Algorithm}[2][tbh]%
%{\begin{myalgo}[#1]
%\centering
%\begin{minipage}{#2}
%\begin{algorithm}[H]}%
%{\end{algorithm}
%\end{minipage}
%\end{myalgo}
%}
%\newcounter{Algo}
%\floatstyle{plain}
%\newfloat{myalgo}{tbhp}{mya}
%
%\newenvironment{Algorithm}[2][tbh]%
%{\begin{myalgo}[#1]
%\refstepcounter{Algo}
%\centering
%\begin{minipage}{#2}
%\begin{algorithm}[H]}%
%{\end{algorithm}
%\end{minipage}
%\end{myalgo}}


\newcommand{\MCSP} {\textsc{Max}}%\text{-}\mathsf{CSP}}
\newcommand{\tE}{\tilde{\mathbb{E}}}
% \newcommand{\Span}{\mathsf{Span}}
\newcommand{\tchi}{\tilde{\chi}}
\newcommand{\tv}{\tilde{v}}
% \newcommand{\dist}{\mathsf{dist}}
\newcommand{\cl}{\mathsf{cl}}
\newcommand{\Ball}{\mathsf{Ball}}
\newcommand{\bchi}{\bar{\chi}}
\newcommand{\Proj}{\mathsf{Proj}}
\newcommand{\eg}{e.~g.}
\newcommand{\zon}{\{0,1\}^n}


%\newcommand{\e}{\epsilon}
\newcommand{\pmo}{\{\pm 1\}}
%\newcommand\Hastad{H{\aa}stad }
%\newcommand\cR{\mathcal{R}}
%\newcommand\cD{\mathcal{D}}
%\newcommand\cP{\mathcal{P}}
%\newcommand\pE{\Tilde{\mathbb{E}}}


\newcommand{\rlin}{\textsc{Real}-\textsc{LIN} }
\renewcommand{\int}{\mathsf{int}}

%newly defined stuff
\newcommand{\MaxC}{\textsc{MAX CLIQUE}}
\newcommand{\nchoose}[1]{{{[n]} \choose {#1}}}
\newcommand{\nperm}[1]{ [n, {#1}]}
\newcommand{\sE}{\mathcal{E}}

\DeclareMathOperator{\lex}{lex}

\renewcommand{\top}{\dagger}

\renewcommand{\1}{\mathbf{1}}

\renewcommand{\hat}{\widehat}


\renewcommand{\on}[1]{\tfrac{\binom{\omega}{#1}}{\binom{n}{#1}}}

\newcommand{\hpE}[1]{\hat{\pE[#1]}}

\newcommand{\xor}{\oplus}

\renewcommand{\emptyset}{\varnothing}



\makeatletter
\let\orgdescriptionlabel\descriptionlabel
\renewcommand*{\descriptionlabel}[1]{%
  \let\orglabel\label
  \let\label\@gobble
  \phantomsection
  \edef\@currentlabel{#1}%
  %\edef\@currentlabelname{#1}%
  \let\label\orglabel
  \orgdescriptionlabel{#1}%
}
\makeatother


%Macros from previous main file.
\newcommand{\gtn}{g^{\otimes n}}
\newcommand{\gtni}{{g^{\otimes n}}^{-1}}
\newcommand{\mnote}[1]{}
\newcommand{\degp}{\mathsf{deg}_{+}}
 \newcommand{\newref}[2][]{\hyperref[#2]{#1~\ref*{#2}}}
\newcommand{\aref}[1]{\newref[Appendix]{#1}}
\newcommand{\sref}[1]{\newref[Section]{#1}}
\newcommand{\dref}[1]{\newref[Definition]{#1}}
\newcommand{\tref}[1]{\newref[Theorem]{#1}}
\newcommand{\lref}[1]{\newref[Lemma]{#1}}
%\newcommand{\pref}[1]{\newref[Proposition]{prop:#1}}
%\newcommand{\cref}[1]{\newref[Corollary]{#1}}
\newcommand{\fref}[1]{\newref[Figure]{fig:#1}}
\newcommand{\rref}[1]{\newref[Remark]{rem:#1}}
\newcommand{\eref}[1]{\newref[Equation]{#1}}
\newcommand{\tbref}[1]{\newref[Table]{#1}}
\newcommand{\clref}[1]{\newref[Claim]{#1}}
\newcommand{\fctref}[1]{\newref[Fact]{#1}}
\renewcommand{\eqref}[1]{\hyperref[#1]{(\ref*{#1})}}
%\newcommand{\opt}{\mathsf{opt}}




\usepackage{latexsym}

%\usepackage{indentfirst}
%\usepackage{makeidx}
%\usepackage{hyperref}


\usepackage{dsfont}
%\usepackage{times}
\usepackage{color}
\usepackage{tikz}

%\renewcommand{\algorithmicrequire}{}

\definecolor{corlinks}{RGB}{64,128,128}
\definecolor{cormenu}{RGB}{0,37,94}
\definecolor{corurl}{RGB}{0,46,91}


%%%Paper specific commands.
\newcommand{\cy}{\mathsf{C}}
\newcommand{\dg}{\mathsf{D}}
\newcommand{\bch}{\mathbb{B}}
\newcommand{\cals}{\mathcal{S}}
\newcommand{\calp}{\mathcal{P}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\gd}{\mc{N}^d}
\newcommand{\sg}{\phi}
\newcommand{\sgg}{\sg_G}
\newcommand{\sgh}{\sg_H}
\newcommand{\sgs}{\sg_S}

\newcommand{\pcg}{\mathsf{PC}_>}
\newcommand{\pd}{\mathcal{P}(n,d)}
\newcommand{\pcgd}{\mathsf{PC}_>(d)}
\newcommand{\ps}{\mathsf{PS}}
\newcommand{\psd}{\mathsf{PS}(d)}
\newcommand{\cali}{\mathcal{I}}

\newcommand{\bd}{\textsc{blockwise-dense }}
\newcommand{\cbd}{\textsc{CBD} }


%Standard notations
%\DeclareMathOperator*{\pr}{\mathsf{Pr}}
%\DeclareMathOperator*{\Var}{\mathsf{Var}}
\renewcommand{\iff}{\Leftrightarrow}
%\DeclareMathOperator*{\ex}{\mathbb{E}}
\newcommand{\rgta}{\rightarrow}
\newcommand{\lfta}{\leftarrow}
%\newcommand{\iprod}[2]{\langle #1,#2\rangle}
\renewcommand{\cal}[1]{\mathcal{#1}}
%\newcommand{\cQ}{\mathcal{Q}}

\newcommand{\inp}[1]{\inpw#1}
\def\inpw#1,#2{\langle #1, #2\rangle}

\newcommand{\cdf}{\mathsf{CDF}}

%\newcommand{\nchoose}[1]{{{[n]} \choose {#1}}}
\newcommand{\nnr}{\mathsf{nnr}}


\renewcommand{\nnr}{\mathsf{rank}_+}
\newcommand{\SA}{\mathsf{SA}}
\newcommand*{\trsp}{\mkern-1mu\intercal}
\newcommand{\err}{\mathsf{err}}

\newcommand{\Dec}{\textsc{Decompose }}
\newcommand{\YDec}{\textsc{YDecompose }}
\newcommand{\XDec}{\textsc{XDecompose }}
\newcommand{\Errord}{\mathsf{Error}_d}
\newcommand{\Errorb}{\mathsf{Error}_b}
\newcommand{\Errora}{\mathsf{Error}_a}
\newcommand{\Error}{\mathsf{Error}}
\renewcommand{\bar}[1]{\overline{#1}}

